Neural Quality Estimation with Multiple Hypotheses for Grammatical Error Correction

Grammatical Error Correction (GEC) aims to correct writing errors and help language learners improve their writing skills. However, existing GEC models tend to produce spurious corrections or fail to detect lots of errors. The quality estimation model is necessary to ensure learners get accurate GEC results and avoid misleading from poorly corrected sentences. Well-trained GEC models can generate several high-quality hypotheses through decoding, such as beam search, which provide valuable GEC evidence and can be used to evaluate GEC quality. However, existing models neglect the possible GEC evidence from different hypotheses. This paper presents the Neural Verification Network (VERNet) for GEC quality estimation with multiple hypotheses. VERNet establishes interactions among hypotheses with a reasoning graph and conducts two kinds of attention mechanisms to propagate GEC evidence to verify the quality of generated hypotheses. Our experiments on four GEC datasets show that VERNet achieves state-of-the-art grammatical error detection performance, achieves the best quality estimation results, and significantly improves GEC performance by reranking hypotheses. All data and source codes are available at https://github.com/thunlp/VERNet.

==> figure/weight.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.90\linewidth]{image/weight.pdf}
    \caption{Ranking Feature Contributions of BERT-ALL.}
    \label{fig:weight}
\end{figure}

==> table/case.tex <==
\begin{table*}[h]
\centering
\small
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{l|l}
\hline


\textbf{\#1 Source}          & The notion of authority also extended 'vertically' . \\ \hline
Basic GEC Model & The notion of authority also extended \textbf{\textcolor{red}{to}} 'vertically' . \\
BERT-VERNet$^{\dagger}$    &  The notion of authority also extended 'vertically' . \\
ELECTRA-VERNet$^{\dagger}$    &  The notion of authority also extended 'vertically' . \\
Golden0 &  The notion of authority also \textbf{\textcolor{red}{extends}} 'vertically' .
\\
Golden1 &  The notion of authority also extended 'vertically' .\\\hline

%\textbf{\#2 Source}          & It can help us know more about each other . \\ \hline
%Baseline & It can help us \textbf{\textcolor{red}{to}} know more about each other . \\
%VERNet    &  It can help us know more about each other . \\ 
%Golden0 & It can help us know more about each other .\\
%Golden1 & \textbf{\textcolor{red}{They}} help us know more about each other .\\\hline

\textbf{\#2 Source}          & It is not a heavy job for the family if they have prepare their mental first by disclosing the information ...\\ \hline
Basic GEC Model & It is not a heavy job for the family if they have \textbf{\textcolor{red}{to}} prepare their \textbf{\textcolor{red}{minds}} first by disclosing the information ... \\
BERT-VERNet$^{\dagger}$    & It is not a heavy job for the family if they have \textbf{\textcolor{red}{prepared}} their \textbf{\textcolor{red}{minds}} first by disclosing the information ... \\ 
ELECTRA-VERNet$^{\dagger}$ & It is not a heavy job for the family if they have \textbf{\textcolor{red}{prepared}} their \textbf{\textcolor{red}{minds}} first by disclosing the information ... \\
Golden0 &  It is not a heavy job for the family if they have \textbf{\textcolor{red}{prepared}} \sout{their} \textbf{\textcolor{red}{mentally}} first by disclosing the information ... \\
Golden1 &  It is not a \textbf{\textcolor{red}{difficult}} job for the family if they have  \textbf{\textcolor{red}{prepared}} their \textbf{\textcolor{red}{minds}} first by disclosing the information ... \\
\hline
\textbf{\#3 Source} & Many of them are busy in work and separate with their children .\\ \hline
Basic GEC Mode & Many of them are busy \textbf{\textcolor{red}{at}} work and separate \textbf{\textcolor{red}{from}} their children .\\
BERT-VERNet$^{\dagger}$ & Many of them are busy \textbf{\textcolor{red}{at}} work and separate \textbf{\textcolor{red}{from}} their children . \\
ELECTRA-VERNet$^{\dagger}$ & Many of them are busy \textbf{\textcolor{red}{at}} work and \textbf{\textcolor{red}{separated from}} their children . \\
Golden0 & Many of them are busy in \textbf{\textcolor{red}{working}} and \textbf{\textcolor{red}{separated}} with their children . \\
Golden1 & Many of them are busy in work and \textbf{\textcolor{red}{separated from}} their children .\\\hline
\end{tabular}}
\caption{\label{tab:case} Cases Generated by Different Models. Three cases are selected from CoNLL-2014. The edited words are \textbf{\textcolor{red}{emphasized}} and the deleted ones are \sout{annotated}.}
\end{table*}

==> table/rerank_all.tex <==
\begin{table*}
\small
\begin{center}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{l| p{0.55cm}<{\centering} p{0.55cm}<{\centering} p{0.55cm}<{\centering} |p{0.55cm}<{\centering} p{0.55cm}<{\centering} p{0.55cm}<{\centering} | p{0.55cm}<{\centering} p{0.55cm}<{\centering} p{0.55cm}<{\centering} | p{0.55cm}<{\centering} p{0.55cm}<{\centering} p{0.55cm}<{\centering} | p{0.7cm}<{\centering}}
\hline \multirow{2}{*}{Model} &  \multicolumn{3}{c|}{CoNLL-2014 (M$^2$)} & \multicolumn{3}{c|}{CoNLL-2014} &  \multicolumn{3}{c|}{FCE} &
\multicolumn{3}{c|}{BEA19} & JFLEG\\ \cline{2-14}
& P & R & F$_{0.5}$ & P & R & F$_{0.5}$ & P & R & F$_{0.5}$ & P & R & F$_{0.5}$ & GLEU\\ \hline
Basic GEC Model & 68.59 & 44.87 & 62.03 & 64.26 & 43.59 & 58.69 & 55.11 & 41.61 & 51.75 & 66.20 & 61.48 & 65.20 & 61.00  \\ 
\hline
BERT-VERNet$^{\dagger}$ (Top2) &  70.93 & \textbf{42.87} & 62.72 & 66.71 & \textbf{41.38} & \textbf{59.43} & 58.59 & \textbf{41.06} & 53.99 & 68.77 & \textbf{60.00} & 66.81 & 61.17  \\ 
BERT-VERNet$^{\dagger}$ (Top3) & 71.97 & 42.01 & \textbf{62.99} & 67.39 & 40.32 & 59.41 & 59.61 & 40.82 & 54.59 & 69.98 & 59.82 & 67.69 & \textbf{61.18} \\ 
BERT-VERNet$^{\dagger}$ (Top4) & \textbf{71.99} & 41.35 & 62.70 & 67.54 & 39.57 & 59.17 & 60.89 & 40.87 & \textbf{55.46} & \textbf{70.42} & 59.53 & \textbf{67.93} & 61.12\\ 
BERT-VERNet$^{\dagger}$ (Top5) & 71.91 & 40.90 & 62.44 & \textbf{67.62} & 39.23 & 59.07 & \textbf{60.97} & 40.69 & 55.44 & 70.19 & 59.21 & 67.68 & 61.06 \\ 
\hline
BERT-ALL (Top2) & 70.89 & \textbf{42.21} & 62.41 & 66.75 & \textbf{40.78} & 59.21 & 58.21 & 41.61 & 53.91 & 69.09 & \textbf{60.35} & 67.15 & 61.47 \\ 
BERT-ALL (Top3) & 72.31 & 41.17 & \textbf{62.80} & 67.85 & 39.39 & 59.28 & 59.33 & \textbf{41.88} & 54.76 & 70.12 & 60.31 & 67.91 & 61.72 \\ 
BERT-ALL (Top4) & 72.43 & 40.65 & 62.64 & \textbf{68.39} & 39.01 & \textbf{59.44} & \textbf{59.92} & 41.83 & \textbf{55.15} & \textbf{70.40} & 60.08 & \textbf{68.06} & 61.84 \\ 
BERT-ALL (Top5) & \textbf{72.53} & 40.19 & 62.48 & 68.28 & 38.67 & 59.21 & \textbf{59.92} & 41.75 & 55.12 & 69.97 & 59.55 &  67.60 & \textbf{61.90} \\
\hline
\end{tabular}}
\caption{\label{tab:beam_rank_all}Performance of Hypothesis Reranking. BERT-VERNet$^{\dagger}$ and BERT-ALL denote adding BERT-VERNet feature and all BERT-based reranking features (BERT-LM, BERT-GQE, BERT-QE, BERT-GED and BERT-VERNet) for reranking.}
\end{center}
\end{table*}
